A View-based Programmable Architecture for Controlling and Integrating Decentralized Data

The view and the view update are known mechanism for controlling access of data and for integrating data of different schemas. Despite intensive and long research on them in both the database community and the programming language community, we are facing difficulties to use them in practice. The main reason is that we are lacking of control over the view update strategy to deal with inherited ambiguity of view update for a given view. This vision paper aims to provide a new language-based approach to controlling and integrating decentralized data based on the view, and establish a software foundation for systematic construction of such data management systems. Our key observation is that a view should be defined through a view update strategy rather than a query. In other words, the view definition should be extracted from the view update strategy, which is in sharp contrast to the traditional approaches where the view update strategy is derived from the view definition. In this paper, we present the first programmable architecture with a declarative language for specifying update strategies over views, whose unique view definition can be automatically derived, and show how it can be effectively used to control data access, integrate data generally allowing coexistence of GAV (global as view) and LAV (local as view), and perform both analysis and updates on the integrated data. We demonstrate its usefulness through development of a privacy-preserving ride-sharing alliance system, discuss its application scope, and highlight future challenges.

==> Incrementalization.tex <==
\subsection{From View Update Specification to Efficient Bidiectional Update Propagation}

\hu{Nakano-seisei: Can you show how to go from the view update description in the language in Section \ref{sec:langugae} to two update propagations; one from view to source and one from source to view. The idea is that we first derive a query from the view update description and the incrementalize both the query and the view update. After that, we may discuss how to improve efficiency by pushdown optimization.}

\subsubsection*{Optimization}
As in ordinary data integration,
several optimization techniques can be considered
for our bidirectional update language.
%In this subsection,
%we discuss on possible optimization

%\paragraph{Push-down optimization}
When processing a query for distributed data among many database servers,
it would be better to avoid redundant data communications
that do not contribute to the result of the query.
%
\newcommand\Bx[1]{\lstinline[basicstyle=\ttfamily,breaklines=true,breakatwhitespace=true]{#1}}
For example,
consider two databases
\Bx{Movie(title, year)} and
\Bx{Director(title, first_name, last_name)}
%\verb|Movie(title, year)| and
%\verb|Director(title, first_name, last_name)|
shown in Section~\ref{sec:bxupdate}
%one includes movies with their titles and published year,
%another includes directors with the titles of their films and
%whose schemas are
and a query for collecting all movies which has a title containing ``love''
and published before 1970.
Although the query can be easily described by joining two databases and
selecting movies satisfying the condition from them,
it is not efficient because many irrelevant data are joined.
The idea of push-down optimization moves selection phases before the join
where both database servers only transmit data of ``love''-titled movies
and particularly the movie server transmits data only before 1970.
PostgreSQL FDW provides push-down optimization for aggregation and join.

Push-down optimization can be considered
not only for view computation but also for view updating.
For an updated view given,
we should reduce the size of a view
to be sent to each source database server.
\todo{In our bidirectional update language,
there is no room for pushdown optimization
because joining tables is allowed only at the top level of queries
(after selection)...}
%the following transformation can be used this optimization:
%\begin{quote}
%\Bx{UPDATE SOURCE} ... \Bx{WHERE} $p$
%\end{quote}
%this can be




==> application.tex <==
\chapter{Applications}

This chapter is to illustrate the power of the programmable architecture with more potential applications.

\hu{Task for the application team.}


\section{Integration of Data for Selling}

There is a synchronization between the view for data buyers and those source data to be sold by data contributors.

\subsubsection{Distribution of Profit for Selling Database Query Answers\protect\footnote{Actually, I don't know this scenario is whether LAV, GAV or LAV/GAV.}}




\begin{figure}[t]
\begin{center}
\begin{small}
\begin{tabular}[t]{|c|c|c|l|l}
\multicolumn{5}{l}{$R_1$}\\
\cline{1-4}
id & time & a\_type & location &\\
\cline{1-4}
 1 & 10:00 & B & Oike & $t_1$\\
 1 & 10:30 & S & Chionin & $t_2$\\
 1 & 11:00 & S & Yasaka & $t_3$\\
 1 & 11:30 & D & Gion & $t_4$\\
\cdashline{1-4}
 1 & 12:00 & D & Gion & $t_5$\\
\cline{1-4}
\end{tabular}
\hspace*{0.5em}
\begin{tabular}[t]{|c|c|c|l|l}
\multicolumn{5}{l}{$R_2$}\\
\cline{1-4}
id & time & a\_type & location &\\
\cline{1-4}
101 & 10:00 & B & Oike & $t_6$\\
101 & 11:00 & B & Oike & $t_7$\\
\cdashline{1-4}
101 & 12:00 & D & Sanjo & $t_8$\\
\cline{1-4}
\end{tabular}
\end{small}
\end{center}
\caption{Personal trajectory data.}
\label{figure:pdm}
\end{figure}


Let us consider two data owners
$u_1$ and $u_2$ who have their respective personal trajectory table
data $R_1$ and $R_2$ shown in Figure~\ref{figure:pdm}.
In these tables, a\_type shows the area type of loations 
(e.g. B(usiness), S(ighseeing) or D(owntown).)
Each personal trajectory table consists of two parts:
{\em public} and {\em private}.
We assume data owners are willing to sell only public data.
Private data is used for data owners' personal purpose.
In our example, we assume the tuples $t_5$ and $t_8$ are private data
whereas all other tuples are public 
(i.e., the tuples above (and below, resp.) the dashed lines in the tables
are pubic (private, resp.).) 


Data buyers specifies the set of data of his/her interest by issuing a query
against a global schema\footnote{It is natural to assume some attributes
can be used only as a target or a qualification in queries. For example, the
{\tt id} in the global schema will not be allowed to appear in 
the target attributes to protect privacy.} 
$$
{\tt G(id, time, a\_type, location).}
$$
Assume a data buyer is interested in the following data:
\begin{quotation}
\noindent
``(time location) pairs of trajectory data of 
users whose {\tt id} is less than 101, or
whose {\tt id} is larger than or equal to 101 and {\tt a\_type} is 
a member of the set $\{{\tt B, D}\}$''
\end{quotation}
This query is expressed in Datalog as follows:
$$
\begin{array}[t]{lll}
Ans(time, location) & := & G(id, time, a\_type, location), \ id < 101 \\
Ans(time, location) & := & G(id, time, a\_type, location), \ id \geq 101, \ a\_type=B\\
Ans(time, location) & := & G(id, time, a\_type, location), \ id \geq 101, \ a\_type=D
\end{array}
$$
The above query against the global schema can easily be transformed into
the following query against the source schemas:
$$
\begin{array}[t]{lll}
Ans(time, location) & := & R_1(id, time, a\_type, location)\\
Ans(time, location) & := & R_2(id, time, a\_type, location), \ a\_type = B\\
Ans(time, location) & := & R_2(id, time, a\_type, location), \ a\_type = D
\end{array}
$$
%
\begin{figure}[t]
\begin{center}
\begin{small}
\begin{tabular}[t]{|c|l|l}
\multicolumn{3}{l}{$Ans$}\\
\cline{1-2}
 time & location &\\
\cline{1-2}
 10:00  & Oike & $t_1, t_6$
\\
 10:30  & Chionin & $t_2$
\\
 11:00  & Oike & $t_7$
\\
 11:00  & Yasaka & $t_3$
\\
 11:30  & Gion & $t_4$
\\
\cline{1-2}
\end{tabular}
\end{small}
\end{center}
\caption{Query answer.}
\label{figure:answer}
\end{figure}
%
Figure~\ref{figure:answer} shows the answer of the query.
Remenber that
only public data of data owners' trajectory tables are available for 
data buyers' query.
Tuple identifiers right outside of the answer table indicate the 
{\em lineage tids} which identify tuples of 
original databases from which the answer row was created.

Data buyer pays a certain amount of money to data owner.
An interesting question is how we should distributed the paid money
among data owners. For example, assume the data buyer paid \$30 for 
the query answer in Figure~\ref{figure:answer}.
How this money should be distributed between the data owners
$u_1$ and $u_2$. There are at least two different policy of distribution:
\begin{enumerate}
 \item\label{policy-tuple}
 Each tuple in the answer should be paid equally.
(In our example, we have five tuples in the answer. Hence,
the data owners who have contribution to create one tuple
are equally paid \$6. 
As a result, $u_1$ and $u_2$ are paid \$21 and \$9 in total, respectively.)

 \item\label{policy-lineage}
 Each lineage tid in the answer should be paid equally.
(In our example, we have six lieage tids in the answer. Hence,
the data owners who have contribution to create one lineage tid
are equally paid \$5. 
As a result, $u_1$ and $u_2$ are paid \$20 and \$10 in total, respectively.)
\end{enumerate}




\subsubsection{Negotiation between data owners and data buyers}


Unfortunately, data buyer is not satisfied with this result because
the answer does not contain any data at noon.
The data buyer believes location data at noon is valuable because
people during lunch time tend to spend more money.
In this case, the data buyer can start {\em negotiation} with data owners.
By offering a certain amount of money for purchasing data at noon,
the data buyer gives data owners an incentive to release their private data.
From database point of view, 
we can interpret the action of starting a negotion as an 
insertion of a new imaginary tuple (12:00, $l$) into the answer in 
Figure~\ref{figure:answer} where $l$ is a variable.
Then, this imaginary tuple is ``traced back''
to the source database.
Here, there are several research questions:
\begin{itemize}
 \item Can we precisely trace the inserted tuple back to the source database?
 \item In more practical schenario, we have a large number of data owners.
       Data buyers will want to set a minimum number for the size of
       tuples and/or lineage ids in answers.
       An example requirement is ``I want to have at least 100 pairs
       (12:00, $l$) in the answer.'' There are at least two
       interpretations for this requirement: 100 different locations,
       or 100 different lineage tids for a single location $l$.
 \item How much money should be offered to give
data owners an incentive to release their private data?
(The data buyer should offer more than \$6 (and \$5, resp.) when
the above-mentioned policy \ref{policy-tuple}
(and policy \ref{policy-lineage}, resp.) was employed 
because price of private data is more expensive than that of public data.)
 \item Negotiation maybe includes the cases where data buyers want to imaginary
       delete/change certain tuples from/in a query answer.
 \item ...
\end{itemize}



% \section{DIAS}

% \hu{Task for Shimizu-sensei.}

\input{dias}


\section{Others}

healthcare systems, ..., iBench


==> dias.tex <==

\section{Curation of Scientific Metadata}

% 科学データの管理においては，そのデータがどのようなものかを示すメタデータが重要である．
% ここでは科学データに対するメタデータを科学メタデータ(scientific metadata)と呼ぶことにする．
% 科学メタデータは，一般的に，分野ごとにフォーマットが異なり，また管理している組織も異なる．
% 各分野でメタデータを利用したデータに対する検索システムなどが構築されている．

For the management of scientific data, 
the metadata which explains the data plays an important role. 
Here we call the metadata for scientific data {\it scientific metadata}. 
Generally, scientific metadata is in different formats depending on the target domains, and 
managed by different organizations. 
Data search systems utilizing scientific metadata are developed in each domain. 


% データ分析による知見発見への期待，特に分野をまたいだ統合解析への期待から，
% 様々なデータ(メタデータ)を統合的に管理する取り組みが行われており，
% 例えば，DIAS (Data Integration and Analysis System) \footnote{http://www.diasjp.net/en/} では日本における地球科学に関連するデータのメタデータを収集している\footnote{なおGEOSS Portal ではglobalに地球科学メタデータを収集しており，DIASはそのノードの一つになっている．}．
% 本節ではDIASを例に用いて，科学メタデータの品質管理への応用事例を説明する．

With the growth of interdisciplinary data science, 
there are some projects for integrated management of scientific data and metadata. 
Such projects include DIAS (Data Integration and Analysis System)\footnote{http://www.diasjp.net/en/}, which manages metadata of earth science related fields in Japan. 
In this section, we explain about the application to the curation of scientific metadata 
using DIAS as an example. 


\subsection{Metadata Management at DIAS}

% DIASでは，地球科学に関連する多様なデータセットを管理しており，
% 自らが保有するデータに関してメタデータを作成すると供に，
% 関連する分野のデータに関して
% 科学メタデータをDIAS外からインポートして統合検索するシステムを構築している．

DIAS manages various datasets concerning earth science, and 
makes the scientific metadata of the datasets stored in the storage of DIAS. 
It also develops the integrated search system called DIAS dataset search and discovery system\footnote{http://search.diasjp.net/en} which is based on the scientific metadata of DIAS and the imported metadata from outside of DIAS. 


\subsubsection{DIAS Dataset Metadata}

% DIASでは保有する全てのデータセットに対して
% データセット単位でメタデータを作成している．
% 多様なデータセットへの適用可能性を意識して，
% データセット名，作成者，概要，時間・空間情報，キーワードなどの
% データセットの概観情報を扱っており，
% ISO 19139の標準に準拠した形式でメタデータを作成している．
% 
% 作成されたメタデータはDIASデータ俯瞰・検索システム \footnote{http://search.diasjp.net/en} を通して
% 閲覧可能になっている．

DIAS makes dataset-level metadata for all datasets. 
As there are various datasets, the metadata is designed to describe 
the overview of the dataset such as dataset name, dataset creator, abstract text, 
spatiotemporal information, keywords, and so on. 
The format of the DIAS dataset metadata is ISO 19139. 
We can browse the metadata through the DIAS dataset search and discovery system. 

% MEMO メタデータに関する言葉の統一感がないかもしれない

% MEMO DOIが付いているデータセットもあり https://doi.org/10.20783/DIAS.496 など

\subsubsection{Metadata Collaboration}

% DIASは地球観測データに関する総合的な検索サイトとしての役割を推進することを目標の一つにしており，
% 特に日本国内における地球観測データの科学メタデータを収集している．
% 
% DIASデータ俯瞰・検索システムでは，いくつかの関連するシステムから科学メタデータをインポートし，
% DIASの科学メタデータと合わせて，統合検索する機能を提供している．
% 図\ref{fig:dias_system_architecture}に連携システムとの関連を示す．
% また，表\ref{tbl:dias_collaborative_systems}に対象となっている連携システムを示す．

One of the function of DIAS is to be a hub of the datasets related to earth science, and 
it is collecting scientific metadata of earth observation datasets especially in Japan. 
The DIAS dataset search and discovery system imports scientific metadata 
from some collaborative systems outside of DIAS, and provides integrated search across systems. 
Figure \ref{fig:dias_system_architecture} shows the relationships with the collaborative systems, and Table \ref{tbl:dias_collaborative_systems} shows the list of collaborative systems. 


% 図\ref{fig:dias_system_architecture}において，
% DIASメタデータ管理システムはDIASにおいてメタデータの作成と管理を担うシステムであり，
% 他の連携システムと同様に，DIASデータ俯瞰・検索システムへメタデータを提供する
% 一システムであるとみなすこともできる．
% また，DIASデータ俯瞰・検索システムは，
% ユーザからの問合せに対する検索結果に連携システムの科学メタデータが含まれる場合，
% 元の連携システムへ誘導するリンクを提供する機能を備えている．

The DIAS metadata management system in Figure \ref{fig:dias_system_architecture} is the system 
for making and managing dataset metadata in DIAS, and can be seen as one of the systems to 
provide metadata to the DIAS dataset search and discovery system along with the collaborative systems. 
Note that the DIAS dataset search and discovery system shows the links to the original information when the search results of queries from users contain scientific metadata from the collaborative systems. 

% MEMO 異なるフォーマットのメタデータをどのように扱っているかの話が必要？
%      現状はかなりad-hoc


\begin{figure}
\centering
\includegraphics[width=8.0cm]{dias_system_architecture.eps}
\caption{Architecture of the DIAS dataset search and discovery system.}
\label{fig:dias_system_architecture}
\end{figure}

\begin{table}
\centering
\caption{Collaborative systems.}
\label{tbl:dias_collaborative_systems}
\begin{tabular}{ll}
System name & Metadata format \\ 
\hline
JAMSTEC Data Catalog			 & DIF \\ 
JaLTER Data Catalog				 & EML \\ 
NIPR Science Database			 & DIF \\ 
NIPR Arctic Data archive System	 & ISO19139, DIF \\ 
\end{tabular}
\end{table}


\subsection{Metadata Quality Issues}

Each scientific metadata is basically created by a different metadata author, 
who is typically a dataset creater or his/her colleague. 
We can observe the manner of writing and the level of detail are different 
depending on metadata author, 
especially for the fields of free description, such as abstract text. 
Also, sometimes we can find fluctuations of description across metadata. 
% 
In addition, when we need to manage metadata in different formats, in such a case like 
metadata collaboration at DIAS, the metadata may contain different types of information. 


To provide proper information to users, and to achieve better findability 
of datasets via the search system, it is important to care about the metadata quality. 
We need much effort to improve the contents of metadata and to keep metadata up to date. 


\subsection{Possible Scenarios}

% メタデータの質を考慮して編集するためには，データベース内の他のメタデータを参照することが
% 重要であると思われる．
% また，更新箇所が多い場合や更新対象となるメタデータの数が多い場合は
% 効率的に編集できることが期待される．
% 
% BXの考え方を用いることで効果的かつ効率的な科学メタデータの品質管理を行うことを検討する．

% TODO ちょっと議論が適当なので改善できないか検討

When we edit metadata with consideration for its quality, 
referring to other metadata seems to be important. 
Also, when we have many parts to be updated, we would like to edit in an efficient way. 
% 
We are considering to utilize the concept of BX 
for effective and efficient curation of scientific metadata. 


\subsubsection{Scenario 1: Focused Editing}

It may be easier for metadata authors to edit metadata 
if they can browse only the focused parts of metadata. 
% 
Getting specific parts in scientific metadata may help finding fluctuation of description. 
For example, by getting elements for the organization name of the dataset creator of each dataset, 
we will be able to find fluctuation of description like 
``Kyoto University'', ``Kyoto Univ.'', and ``KU'', 
which should be unified and tend to be missed out when we browse whole metadata. 

% TODO まだ言葉が足りていない感
% TODO 図を作る


\subsubsection{Scenario 2: Bulk Editing}

Sometimes, we would like to update all occurrences of the same value or same element. 
% 
For example, when a contact personnel who is in charge of multiple datasets changes, 
we need to edit all contact information of his/her datasets. 
By getting aggregated elements for the contact information, 
we can simultaneously edit all occurrences of his/her name. 

% TODO まだ言葉が足りていない感
% TOOD 図を作る




% MEMO ひとまず熱海合宿発表内容＋調整まで

% TODO もっといろんな状況をモデル化したい(合宿での議論がまだ十分には反映できていない)
% TODO どこがmaterializedされているのかといった意識を踏まえた議論

% TODO 特にメタデータ連携している場合はメタデータのフォーマットが多様になりえるが、
%      そのような話がシナリオにあまり生かされていない




==> runningExample.tex <==

\chapter{Running Example: Ride-Sharing Systems}
\label{ch:runningExample}

%This chapter will explain the requirement/specification of a ride-sharing system, which will be served as the running example of this technical report. We will show the limitation of the existing techniques in implementing such such system, and highlight what we can do.

\hu{Task for Asano-sensei and Tsushima-sensei.}

\section{Current Ride-Sharing Systems}

%%ライドシェアリングの普及
%% ride-sharing (ridesharingの方が多かった)

%def. of or relating to a car service with which a person uses a smartphone app to arrange a ride in a usually privately owned vehicle.
%Essentially, UBER. Ridesharing can mean the use of services like Liftshare through their iOS or Android apps, but is normally used when referring to an on-demand service – making it a taxi.

Recently, it has attracted the attention that ``ride-sharing'' which allows a person other than professional taxi drivers to provide a car service using his/her privately owned vehicle, as an effective approach for reducing traffic jams and improving an environment. 
Uber and Lyft are representative ride-sharing services. 
Lyft provides conventional transportation services in addition to the ride-sharing, while they reported that ride-sharing occupies over $40\%$ of their all requests in 2016.



%Carsharing
%def. the practice of sharing a car for regular travelling, especially for commuting.
%Carsharing is sharing spare seats in vehicles with those who are going the same way, either on a one-off or regular basis – and can be to and from anywhere. This may be through a matching service like Liftshare, or an informal arrangement between friends. There may be money exchanged, alternating driving arrangements made, or it can be completed as a favour. Interestingly, this is what ‘carpooling’ means in the rest of the world outside of the UK!

%%ライドシェアリングのモデル

There are various service models for ride-sharing. 
The following description explains criteria for classifying the ride-sharing service models. 

\begin{itemize}
	\item Whether driver's own destination exists: Some models assume that, as each driver moves to his/her own destination, he/she also carries passengers. On the other hand, most commercial services assume that every driver has no own destination and waits a request from a passenger as well as taxis do. 
	\item Whether multiple passenger groups are allowed (carpooling): Conventional models do not allow a taxi to pick up a new passenger until it reaches the destination of the current passenger. However, if a model allows to do so, then several advantages might be obtained; for example, a fee per passenger can be reduced or the total mileage can be reduced. Uber is experimentally operating such a service.
	\item Static or dynamic: Most theoretical researches of ride-sharing have adopted static models for matching drivers and passengers. 
	The objective of static models is to compute an optimal matching for all requests given in advance. Furuhata et al.~\cite{furuhata2013ridesharing} conducted a comprehensive study on formalization and optimization for various static ride-sharing models.  Santi et al.~\cite{santi2014quantifying} quantified the potential of ride-sharing by applying a graph theory based approach to New York taxi data. 
    %Cici et al.~\cite{cici2014assessing} evaluated the potential of carpooling using a dataset of actual requests on four cities. 
	On the other hand, ride-sharing services utilizing mobile applications, such as Uber and Lyft, match a passenger and a driver dynamically (in real-time) whenever a request from a passenger comes. 
    %Santos et al.~\cite{santos2013dynamic} proposed a ride-sharing system to maximize the number of matched requests. 
    Ma et al.~\cite{ma2013t}\cite{ma2015real} proposed a method named ``T-share'' for dynamic matching which minimizes drivers' total mileage.
    %This method employs a spatial-temporal index to retrieve candidate drivers efficiently. 
    Huang \cite{huang2014large} proposed a data structure ``kinect tree'' for managing the pick-up and drop-off schedule of each driver, and proposed an algorithm finding a matching with the minimum increase of total mileage. 
    Ota et al.~\cite{ota2015scalable} introduced a data-driven simulation framework that enables the analysis of ride-sharing by using New York taxi dataset.
	\item Whether detours are allowed: In a model allowing carpooling, a vehicle might not be able to follow the shortest path for a passenger if it wants to pick up another passenger before it arrives the destination of the first passenger. Such a case is called a detour. If a model does not allow a detour, a vehicle must follow the shortest path always for current passengers. 
	\item Direct or indirect journey: In a direct journey model, driver picks up a passenger at his/her departure place (sometimes the home) and drops off him/her at his/her destination. In this model, it is difficult for passengers to conceal their important locations to drivers. 
    In an indirect journey model, the pick-up (and drop-off) point can be different from the departure place (and destination, respectively). 
	\item Objective function: Candidates include minimization of total mileage, maximization of the benefit of a system, and maximization of the number of matchings. 
\end{itemize}


%ライドシェアリングのプライバシーまたは機密情報保護
As ride-sharing becomes popular, protecting the privacy of passengers and drivers have become a problem.  
Because drivers are not professional in ride-sharing, passengers might not disclose their important locations to many drivers, and vice versa. 
There is a few researches which tackled with this problem. 
\begin{itemize}
	\item Aïvodji et al.~\cite{aivodji2016privacy} proposed a method for computing an indirect journey for  a driver and a passenger without disclosing their precise locations by employing a homomorphism. Unfortunately, their method does not consider practical ride-sharing which requires to compute a matching among multiple drivers and passengers. 
   \item Goel et al.~\cite{goel2016privacy} proposed a method for matching drivers and passengers for direct journeys and reducing the number of drivers and passengers who know the precise locations of others by approximating location information. This method employs a review system in order to eliminate malicious drivers or passengers instead of preventing their attacks directly. 
	\item Tong et al.~\cite{tong2017privacy} proposed a method utilizing differential privacy which have been known as a powerful technique for protecting privacy recently. This method does not support an indirect journey. 
\end{itemize}
%まだ，間接行程の研究はほとんどない



\section{Future Ride-Sharing Systems}

%我々のやろうとしていること
As companies who want to enter into the ride-sharing market increase, it is expected that alliances between companies also increase. 
%Note that such an alliance might accept not only companies but also a person or a family as a participant.   
A system for realizing an alliance of ride-sharing companies might assume that an mediator (a third party, trusted in some degree) receives requests from passengers and matches each request to a vehicle belonging to one of the companies. 
Although the privacy of passengers and the secret information of companies would be a problem, the previous privacy-preserving ride-sharing methods introduced above cannot deal with this problem. 
We tackle with this problem in this paper. 

A passenger would want to reduce the number of companies who know his/her precise pick-up/drop-off locations. 
A company would not want to send the precise locations of persons who are registered as drivers to the company. 
Therefore, it would be required a framework that the mediator collects approximate location data of vehicles, estimates the best vehicle for each request using the data, and sends the precise location of the passenger to the company having the vehicle. 
In such a framework, because the estimation is based on approximate locations, the obtained vehicle might not be the best one based on its precise location.  
For example, it is possible that the estimated benefit for a request is positive but its precise benefit is negative, or the estimated arrival time can be far from the precise one. 
Because drivers are not professional in ride-sharing service, the company might have a policy not to accept a request with insufficient benefit. 
In addition, acceptance policies for requests can be different among companies.

The following framework is one of the possible solutions. 
\begin{enumerate}
	\item Each company sends approximate locations of vehicles belonging to the company to the mediator. 
   \item The mediator integrates the data of all companies, and then generates a ranking of vehicles for a given request based on various criteria such as the estimated benefit of the system and the estimated arrival time. 
   \item The mediator repeats the procedures below until the matching of a vehicle and the request is fixed.
   \begin{enumerate}
		\item The mediator obtain the top vehicle of the ranking, and send the request and the precise location of the passenger to the company who manages the vehicle. 
		\item The company computes the precise benefit and arrival time based on the precise locations of the vehicles and passengers, and decide whether the company accepts the request based on the company policy (for example, the company will not accept a request if its benefit is negative or its arrival time is too late for the passenger). 
		\item If the request is accepted, then the mediator fixes the matching for the request. After that, the company processes the request (picks the passenger up). 
	   \item Otherwise, the mediator deletes the vehicle from the ranking (and go back to the step (3.a)).
   \end{enumerate}
\end{enumerate}
%(1) 得られたリストの上からタクシーの予約を該当するpeerにupdate文を用いて要求
%(2) peerは，(peerのローカルな情報を使って要求を受け入れるかどうかを決定) 
%　　　受け入れるなら，与えられたupdateをビュー(例えば，Figure 4.1の四角Aの中の下のビュー)に実行
%　　　updateを基底関係(例えば，Figure 4.1の四角Aの中の上の部分)に反映し，OKを返す
%　　　受け入れないなら，その旨をmediatorに通知
%(3) mediatorは，updateがOKならそれで予約終了
%　　　updateが受け入れられないなら，リストの次の候補のタクシーを予約
%(1)から(3)をOKになるまで繰り返す．


The data integration on this framework has to allow each company to update their data according to its policy, keeping the consistency between the approximate location data of the mediator and the precise location data of each company. 
Such an integration is difficult to implement using conventional data integration methods. 
For example, a naive approach that the mediator maintains all the data and the code for managing them is difficult to realize,  because the mediator has to prepare a code specialized to each company with a different policy from the others, and the code 
should need precise location data for checking whether the policy is satisfied.  
%正確な位置情報を秘匿計算で利用する方法はありそう 今回は秘匿計算はなし
Another candidate of approaches for data integration is that the mediator and all companies share the data of all vehicles and requests by utilizing existing data sharing methods including CDSS. 
It is more difficult for this approach to keep the precise locations of vehicles and passengers secret. 
Even if it is possible, each company has to take enormous effort to develop a program for updating its data according to its policy. 
Therefore, a desired approach for implementing the framework above is to enable each company to easily describe which part of its own data should be disclosed to the mediator and how its policy for accepting a request should be. 
In addition, once if such a description is prepared, the approach has to guarantee mediator's data and companies' data to be updated keeping the consistency between the approximate location data of the mediator and the precise location data of each company. 


\section{Updates for Ride-Sharing Systems}

\subsection{Simple ride-sharing}


\begin{figure}
  \includegraphics[width=10.0cm]{./Examples/1.eps}
  \caption{An Example of simple ride-sharing} \label{Simplesharing}
\end{figure}

\begin{figure}
  \includegraphics[width=10.0cm]{./Examples/2.eps}
  \caption{Request by the mediator} \label{Simplesharingtwo}
\end{figure}


\begin{figure}
  \includegraphics[width=10.0cm]{./Examples/3.eps}
  \caption{A taxi moved} \label{Simplesharingthree}
\end{figure}


\begin{figure}
  \includegraphics[width=10.0cm]{./Examples/4.eps}
  \caption{A taxi became empty} \label{Simplesharingfour}
\end{figure}

In the simple ride-sharing, 
we will use the following settings.

\begin{itemize}
\item Companies always accept the request by the mediator.
\item Companies share all of car information with the mediator.
\end{itemize}

Figure \ref{Simplesharing} shows example tables of simple ride-sharing.
In the upper boxes of the figure, there are tables of companies.
The upper tables are internal tables in companies. The lower tables 
are sharing table with the mediator (They are view of the original table).
In this simple setting companies share all of their car information.
Because detailed location information is secret, specific data (Kanda, Shinjyuku, etc.) in the original table are changed rough locations (Tokyo, Kyoto, etc.).

The lower box is mediator's table. It is a simple union of companies views.
Using this example, we can consider the following updates.


\begin{itemize}
\item [(1)] Mediator sends a request (car No., userID and location) to a company.
Because companies always accept the requests, the original table is changed using them. (Fig.\ref{Simplesharingtwo})
\item [(2)] Companies send update information when their taxi's rough location was changed. The mediator table is always changed. (Fig. \ref{Simplesharingthree})

\item [(3)] Companies send update information when one of their taxis become empty
(passengers arrived at their destination). The mediator table is always changed. (Fig. \ref{Simplesharingfour})
\end{itemize}



\subsection{Advanced ride-sharing}

\begin{figure}
  \includegraphics[width=10.0cm]{./Examples/5.eps}
  \caption{An Example of advanced ride-sharing} \label{Adsharing}
\end{figure}

\begin{figure}
  \includegraphics[width=10.0cm]{./Examples/6.eps}
  \caption{Request by the mediator} \label{Adsharingtwo}
\end{figure}


\begin{figure}
  \includegraphics[width=10.0cm]{./Examples/7.eps}
  \caption{A taxi moved} \label{Adsharingthree}
\end{figure}

\begin{figure}
  \includegraphics[width=10.0cm]{./Examples/8.eps}
  \caption{A taxi became empty} \label{Adsharingfour}
\end{figure}

In the advanced ride-sharing,
we will use the following settings. 

\begin{itemize}
\item Companies can reject the request by the mediator. In that case mediator will search other possibilities.
\item Companies share only empty-car information with the mediator.
\end{itemize}

Figure \ref{Adsharing} shows example tables of advanced ride-sharing.
In the advanced ride-sharing companies share only empty-car information.
Therefore shared tables are smaller than the simple ride-sharing.


Using this example, we can consider the following updates.

\begin{itemize}
\item [(1)] Mediator sends a request (car No., userID and location) to a company.
The original table is changed by the request. 
In this case, the car No.2 disappered from the shared table after the original table is changed. This is because the view includes only empty-car information. (Fig.\ref{Adsharingtwo})
\item [(2)] Companies send update information when their taxi's rough location was changed. If it is in the mediator view, the mediator table is changed. Otherwise nothing happens in the mediator view. (Fig.\ref{Adsharingthree})

\item [(3)] Companies send update information when one of their taxis become empty
(passengers arrived at their destination). In the example, a record is added to the mediator view. (Fig.\ref{Adsharingfour})
\end{itemize}

